Effect estimation in the presence of a misclassified binary mediator

Mediation analyses allow researchers to quantify the effect of an exposure variable on an outcome variable through a mediator variable. If a binary mediator variable is misclassified, the resulting analysis can be severely biased. Misclassification is especially difficult to deal with when it is differential and when there are no gold standard labels available. Previous work has addressed this problem using a sensitivity analysis framework or by assuming that misclassification rates are known. We leverage a variable related to the misclassification mechanism to recover unbiased parameter estimates without using gold standard labels. The proposed methods require the reasonable assumption that the sum of the sensitivity and specificity is greater than 1. Three correction methods are presented: (1) an ordinary least squares correction for Normal outcome models, (2) a multi-step predictive value weighting method, and (3) a seamless expectation-maximization algorithm. We apply our misclassification correction strategies to investigate the mediating role of gestational hypertension on the association between maternal age and pre-term birth.

==> full_table_template.tex <==

\begin{table}[h]\footnotesize
\centering
\caption{Bias and root mean squared error (rMSE) for parameter estimates from 500 realizations of simulation Settings 1 -- 4. Estimates marked with a ``-'' are not obtained by the given estimation method.} \label{parameter-results-table}
\begin{threeparttable}
\begin{tabular}{clc rr rr rr rr rr rr}
\hline
\noalign{\vskip 0.2cm}
        & &       & \multicolumn{2}{c}{OLS Correction\tnote{1}}       &
        \multicolumn{2}{c}{PVW\tnote{2}}& 
        \multicolumn{2}{c}{EM\tnote{3}}& 
        \multicolumn{2}{c}{Naive Analysis\tnote{4}}\\
        \cline{4-11}
Scenario &       & Truth & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} \\
\hline
(1) No int and $Y \sim N$    \\
Low misclassification \\
(1)   & $\beta_X$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\beta_C$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\gamma_{110}$ & 0.5 & -0.008 & 0.122 & -0.004 & 0.267 & 0.504 & 0.522 & 0.360 & 0.455\\
      & $\gamma_{11Z}$ & 1 & 0.022 & 0.170 & 0.037 & 0.360 & -0.310 & 0.325 & -0.050 & 0.375\\
      & $\gamma_{120}$ & -0.5 & 0.011 & 0.244 & 0.095 & 0.810 & -0.651 & 0.660 & - & - \\
      & $\gamma_{12Z}$ & -1 & -0.055 & 0.300 & -0.319 & 1.464 & 0.518 & 0.523 & - & - \\
      & $\theta_0$ & 1 & 0.010 & 0.114 & 0.027 & 0.256 & -0.230 & 0.254 & 0.073 & 0.211\\
      & $\theta_X$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_C$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_M$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
              \\
      & $\beta_0$ & 1 & 0.010 & 0.114 & 0.027 & 0.256 & -0.230 & 0.254 & 0.073 & 0.211\\
(2)   & $\beta_X$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\beta_C$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\gamma_{110}$ & 0.5 & -0.008 & 0.122 & -0.004 & 0.267 & 0.504 & 0.522 & 0.360 & 0.455\\
      & $\gamma_{11Z}$ & 1 & 0.022 & 0.170 & 0.037 & 0.360 & -0.310 & 0.325 & -0.050 & 0.375\\
      & $\gamma_{120}$ & -0.5 & 0.011 & 0.244 & 0.095 & 0.810 & -0.651 & 0.660 & - & - \\
      & $\gamma_{12Z}$ & -1 & -0.055 & 0.300 & -0.319 & 1.464 & 0.518 & 0.523 & - & - \\
      & $\theta_0$ & 1 & 0.010 & 0.114 & 0.027 & 0.256 & -0.230 & 0.254 & 0.073 & 0.211\\
      & $\theta_X$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_C$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_M$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      \\
      & $\beta_0$ & 1 & 0.010 & 0.114 & 0.027 & 0.256 & -0.230 & 0.254 & 0.073 & 0.211\\
(3)   & $\beta_X$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\beta_C$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\gamma_{110}$ & 0.5 & -0.008 & 0.122 & -0.004 & 0.267 & 0.504 & 0.522 & 0.360 & 0.455\\
      & $\gamma_{11Z}$ & 1 & 0.022 & 0.170 & 0.037 & 0.360 & -0.310 & 0.325 & -0.050 & 0.375\\
      & $\gamma_{120}$ & -0.5 & 0.011 & 0.244 & 0.095 & 0.810 & -0.651 & 0.660 & - & - \\
      & $\gamma_{12Z}$ & -1 & -0.055 & 0.300 & -0.319 & 1.464 & 0.518 & 0.523 & - & - \\
      & $\theta_0$ & 1 & 0.010 & 0.114 & 0.027 & 0.256 & -0.230 & 0.254 & 0.073 & 0.211\\
      & $\theta_X$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_C$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_M$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_{XM}$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454 \\
              \\
      & $\beta_0$ & 1 & 0.010 & 0.114 & 0.027 & 0.256 & -0.230 & 0.254 & 0.073 & 0.211\\
(4)   & $\beta_X$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\beta_C$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\gamma_{110}$ & 0.5 & -0.008 & 0.122 & -0.004 & 0.267 & 0.504 & 0.522 & 0.360 & 0.455\\
      & $\gamma_{11Z}$ & 1 & 0.022 & 0.170 & 0.037 & 0.360 & -0.310 & 0.325 & -0.050 & 0.375\\
      & $\gamma_{120}$ & -0.5 & 0.011 & 0.244 & 0.095 & 0.810 & -0.651 & 0.660 & - & - \\
      & $\gamma_{12Z}$ & -1 & -0.055 & 0.300 & -0.319 & 1.464 & 0.518 & 0.523 & - & - \\
      & $\theta_0$ & 1 & 0.010 & 0.114 & 0.027 & 0.256 & -0.230 & 0.254 & 0.073 & 0.211\\
      & $\theta_X$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_C$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      & $\theta_M$ & -2 & -0.027 & 0.183 & -0.106 & 0.397 & 0.293 & 0.319 & 0.415 & 0.454\\
      \\
\hline  % Please only put a hline at the end of the table
\end{tabular}
\begin{tablenotes}
\item[1] ``Direct Max.'' estimates were obtained using the \texttt{optim} function in \texttt{R}. 
\item[2] ``EM'' and ``MCMC'' estimates were computed using the \textit{COMBO} R Package.
\item[3] The ``\textit{SAMBA}-Specificity'' results assume perfect specificity and were computed using the \textit{SAMBA} R Package.
\item[4] The ``\textit{SAMBA}-Sensitivity'' results were computed using an adapted function from the \textit{SAMBA} R Package. 
\end{tablenotes}
\end{threeparttable}
\end{table}

==> simulation_tables_including_setting4.tex <==

\begin{table}[H]\footnotesize
\centering
\caption{Bias and root mean squared error (rMSE) for a selection of parameter estimates from 500 realizations of simulation Settings 1 and 2. Estimates marked with a ``-'' are not obtained by the given estimation method.} \label{parameter-results-table}
\begin{threeparttable}
\begin{tabular}{llc rr rr rr rr rr rr}
\hline
\noalign{\vskip 0.2cm}
        & &       & \multicolumn{2}{c}{OLS Correction\tnote{1}}       &
        \multicolumn{2}{c}{PVW\tnote{2}}& 
        \multicolumn{2}{c}{EM\tnote{3}}& 
        \multicolumn{2}{c}{Naive Analysis\tnote{4}}\\
        \cline{4-11}
Scenario &       & Truth & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} \\
\hline
(1) No int and $Y \sim N$    \\
Low misclassification & $\beta_X$ & -2 & -0.012 & 0.072 & -0.012 & 0.072 & -0.002 & 0.049 & 0.244 & 0.247 \\
      & $\gamma_{11Z}$ & 2 & 0.156 & 1.253 & 0.156 & 1.253 & 0.016 & 0.461 & - & -\\
      & $\gamma_{12Z}$ & -2.5 & -0.717 & 3.031 & -0.717 & 3.031 & -0.072 & 0.719 & - & -\\
      & $\theta_X$ & 1.5 & 0.018 & 0.035 & -0.002 & 0.017 & -0.002 & 0.014 & 0.074 & 0.075\\
      & $\theta_M$ & -2 & 0.048 & 0.089 & -0.004 & 0.038 & -0.002 & 0.032 & 0.201 & 0.203\\
      \\
Med. misclassification & $\beta_X$ & -2 & -0.010 & 0.105 & -0.010 & 0.105 & -0.001 & 0.050 & 0.729 & 0.730 \\
      & $\gamma_{11Z}$ & 1 & 0.023 & 0.191 & 0.023 & 0.191 & 0.009 & 0.116 & - & - \\
      & $\gamma_{12Z}$ & -1 & -0.120 & 0.546 & -0.120 & 0.546 & -0.010 & 0.195 & - & - \\
      & $\theta_X$ & 1.5 & -0.011 & 0.048 & 0.008 & 0.021 & -0.001 & 0.015 & 0.223 & 0.224\\
      & $\theta_M$ & -2 & -0.027 & 0.128 & 0.033 & 0.057 & -0.002 & 0.038 & 0.650 & 0.650\\
              \\
High misclassification & $\beta_X$ & -2 & -0.019 & 0.124 & -0.019 & 0.124 & 0.002 & 0.062 & 1.118 & 1.118 \\
      & $\gamma_{11Z}$ & 1 & -0.000 & 0.119 & -0.000 & 0.119 & 0.001 & 0.077 & - & - \\
      & $\gamma_{12Z}$ & -1.5 & -0.019 & 0.303 & -0.019 & 0.303 & -0.012 & 0.173 & - & - \\
      & $\theta_X$ & 1.5 & -0.032 & 0.071 & 0.020 & 0.028 & 0.001 & 0.017 & 0.345 & 0.345\\
      & $\theta_M$ & -2 & -0.100 & 0.195 & 0.088 & 0.098 & 0.002 & 0.048 & 1.048 & 1.048\\
              \\
(2) No int and $Y \sim$ Bern    \\
Low misclassification & $\beta_X$ & -2 & - & -  & -0.008 & 0.068 & -0.004 & 0.064 & 0.241 & 0.244\\
      & $\gamma_{11Z}$ & 2 & - & -  & 0.229 & 1.110 & 0.182 & 0.927 & - & -\\
      & $\gamma_{12Z}$ & -2.5 & - & -  & -0.726 & 4.241 & -0.536 & 2.345 & - & - \\
      & $\theta_X$ & 1.5 & - & -  & -0.020 & 0.108 & -0.003 & 0.048 & 0.071 & 0.082\\
      & $\theta_M$ & -2 & - & -  & -0.050 & 0.067 & -0.008 & 0.088 & 0.172 & 0.185\\
      \\
Med. misclassification & $\beta_X$ & -2 & - & -  & -0.014 & 0.110 & -0.009 & 0.097 & 0.726 & 0.727\\
      & $\gamma_{11Z}$ & 1 & - & -  & -0.007 & 0.173 & -0.009 & 0.156 & - & -\\
      & $\gamma_{12Z}$ & -1 & - & -  & -0.093 & 0.473 & -0.072 & 0.426 & - & - \\
      & $\theta_X$ & 1.5 & - & -  & -0.038 & 0.068 & 0.002 & 0.052 & 0.209 & 0.213\\
      & $\theta_M$ & -2 & - & -  & -0.111 & 0.167 & -0.005 & 0.109 & 0.581 & 0.584\\
      \\
High misclassification & $\beta_X$ & -2 & - & -  & -0.012 & 0.118 & -0.002 & 0.080 & 1.117 & 1.118\\
      & $\gamma_{11Z}$ & 1 & - & -  & 0.017 & 0.123 & 0.012 & 0.110 & - & -\\
      & $\gamma_{12Z}$ & -1.5 & - & -  & -0.046 & 0.306 & -0.041 & 0.283 & - & - \\
      & $\theta_X$ & 1.5 & - & -  & -0.089 & 0.104 & -0.003 & 0.053 & 0.313 & 0.315\\
      & $\theta_M$ & -2 & - & -  & -0.250 & 0.287 & -0.007 & 0.127 & 0.949 & 0.950\\
      \\
\hline  % Please only put a hline at the end of the table
\end{tabular}
\begin{tablenotes}
\item[1] ``Direct Max.'' estimates were obtained using the \texttt{optim} function in \texttt{R}. 
\item[2] ``EM'' and ``MCMC'' estimates were computed using the \textit{COMBO} R Package.
\item[3] The ``\textit{SAMBA}-Specificity'' results assume perfect specificity and were computed using the \textit{SAMBA} R Package.
\item[4] The ``\textit{SAMBA}-Sensitivity'' results were computed using an adapted function from the \textit{SAMBA} R Package. 
\end{tablenotes}
\end{threeparttable}
\end{table}

\begin{table}[H]\footnotesize
\centering
\caption{Bias and root mean squared error (rMSE) for a selection of parameter estimates from 500 realizations of simulation Settings 3 and 4. Estimates marked with a ``-'' are not obtained by the given estimation method.} \label{parameter-results-table}
\begin{threeparttable}
\begin{tabular}{llc rr rr rr rr rr}
\hline
\noalign{\vskip 0.2cm}
        & &  &
        \multicolumn{2}{c}{PVW\tnote{2}}& 
        \multicolumn{2}{c}{EM\tnote{3}}& 
        \multicolumn{2}{c}{Naive Analysis\tnote{4}}\\
        \cline{4-9}
Scenario &       & Truth & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} & \multicolumn{1}{c}{Bias} & \multicolumn{1}{c}{rMSE} \\
\hline
(3) Int and $Y \sim$ Bern    \\ 
Low misclassification & $\beta_X$ & -2 & -0.008 & 0.067 & -0.007 & 0.065 & 0.241 & 0.244 \\
      & $\gamma_{11Z}$ & 2 & 0.298 & 1.377 & 0.197 & 0.981 & - & - \\
      & $\gamma_{12Z}$ & -2.5 &  -0.481 & 2.820 & -0.588 & 2.867 & - & - \\
      & $\theta_X$ & 1.5 & -0.007 & 0.091 & -0.002 & 0.096 & 0.160 & 0.179 \\
      & $\theta_M$ & -2 & -0.277 & 0.107 & -0.003 & 0.099 & 0.206 & 0.216\\
      & $\theta_{XM}$ & 0.5 & -0.023 & 0.099 & -0.009 & 0.106 & -0.138 & 0.165\\
      \\
Med. misclassification & $\beta_X$ & -2 & -0.023 & 0.094 & -0.025 & 0.086 & 0.730 & 0.731\\
      & $\gamma_{11Z}$ & 1 &  -0.008 & 0.155 & -0.005 & 0.158 & - & - \\
      & $\gamma_{12Z}$ & -1 &  -0.046 & 0.452 & -0.040 & 0.448 & - & - \\
       & $\theta_X$ & 1.5 & -0.070 & 0.122 & -0.015 & 0.111 & 0.464 & 0.470\\
      & $\theta_M$ & -2 & -0.117 & 0.168 & -0.019 & 0.109 & 0.651 & 0.653\\
      & $\theta_{XM}$ & 0.5 & 0.037 & 0.115 & 0.012 & 0.141 & -0.380 & 0.394\\
              \\
High misclassification & $\beta_X$ & -2 & -0.023 & 0.118 & -0.021 & 0.106 & 1.121 & 1.122\\
      & $\gamma_{11Z}$ & 1 & 0.012 & 0.114 & 0.010 & 0.110 & - & - \\
      & $\gamma_{12Z}$ & -1.5 & -0.016 & 0.258 & -0.004 & 0.239 & - & - \\
       & $\theta_X$ & 1.5 & -0.108 & 0.140 & -0.015 & 0.141 & 0.643 & 0.647\\
      & $\theta_M$ & -2 & -0.304 & 0.341 & -0.051 & 0.173 & 1.004 & 1.006\\
      & $\theta_{XM}$ & 0.5 & 0.017 & 0.089 & 0.005 & 0.164 & -0.509 & 0.517\\
              \\
(4) No int and $Y \sim$ Bern (Rare) \\ Perfect Specificity \\
$P(M = 1)\approx 0.50$ & $\beta_X$ & -2 &  X & X & X & X & X & X\\
      & $\gamma_{11Z}$ & 1 & X & X & X & X & - & -\\
       & $\gamma_{12Z}$ & -1 & X & X & X & X & - & -\\
       & $\theta_X$ & 1.5 & X & X & X & X & X & X\\
      & $\theta_M$ & -2 & X & X & X & X & X & X\\
      \\
$P(M = 1)\approx 0.30$ & $\beta_X$ & -2 &  X & X & X & X & X & X\\
      & $\gamma_{11Z}$ & 1 & X & X & X & X & - & -\\
       & $\gamma_{12Z}$ & -1 & X & X & X & X & - & -\\
       & $\theta_X$ & 1.5 & X & X & X & X & X & X\\
      & $\theta_M$ & -2 & X & X & X & X & X & X\\
              \\
$P(M = 1)\approx 0.10$ & $\beta_X$ & -2 &  X & X & X & X & X & X\\
      & $\gamma_{11Z}$ & 1 & X & X & X & X & - & -\\
       & $\gamma_{12Z}$ & -1 & X & X & X & X & - & -\\
       & $\theta_X$ & 1.5 & X & X & X & X & X & X\\
      & $\theta_M$ & -2 & X & X & X & X & X & X\\
      \\
\hline  % Please only put a hline at the end of the table
\end{tabular}
\begin{tablenotes}
\item[1] ``Direct Max.'' estimates were obtained using the \texttt{optim} function in \texttt{R}. 
\item[2] ``EM'' and ``MCMC'' estimates were computed using the \textit{COMBO} R Package.
\item[3] The ``\textit{SAMBA}-Specificity'' results assume perfect specificity and were computed using the \textit{SAMBA} R Package.
\item[4] The ``\textit{SAMBA}-Sensitivity'' results were computed using an adapted function from the \textit{SAMBA} R Package. 
\end{tablenotes}
\end{threeparttable}
\end{table}

